Quadrotor Trajectory Tracking Using Linear and Nonlinear Model Predictive Control

Accurate trajectory tracking is an essential characteristic for the safe navigation of a quadrotor in cluttered or disturbed environments. In this paper, we present in detail two state-of-the-art model-based control frameworks for trajectory tracking: the Linear Model Predictive Controller (LMPC) and the Nonlinear Model Predictive Controller (NMPC). Additionally, the kinematic and dynamic models of the quadrotor are comprehensively described. Finally, a simulation system is implemented to verify feasibility, demonstrating the effectiveness of both controllers.

==> vncaps.tex <==
% Copyright 2000-2006 Werner Lemberg <wl@gnu.org> and
%                     Han The Thanh <hanthethanh@gmx.net>.
% This file is part of vntex.  License: LPPL, version 1.3 or newer,
% according to http://www.latex-project.org/lppl.txt

\ifx\ProvidesFile\undefined \else
  \ProvidesFile{vncaps.tex}[2006/06/07 v1.1 Captions in Vietnamese]  
\fi
 
% Vietnamese captions; edit them in viscii/tcvn/utf8, then use
% `vntovn viscii vntex' or a similar command to convert to vntex.
%
% History
%
% ????/??/??:
%     Split off captions from vietnam.ldf.
%     Add \captionsenglish, \dateUSenglish, and \dateenglish.
%
% 2005/04/21:
%     Add copyright message.
%     Don't use `{}' but a space after macros which don't have arguments.
%
% 2006/06/07:
%     Fix bug in \indexname.  Add version number.

\ifx\providecommand \undefined
  \let\providecommand \def
\fi

\providecommand\captionsvietnam{% 
  \def\prefacename{L\`\ohorn i n\'oi \dj\`\acircumflex u}%
%  \def\refname{T\`ai li\d\ecircumflex u}%
  \def\Acknowledgmentname{L\`\ohorn i c\h{a}m \ohorn n}%
  \def\refname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
%  \def\abstractname{T\'om t\'\abreve t n\d\ocircumflex i dung}
  \def\abstractname{T\'om t\'\abreve t}
  \def\IEEEkeywordsname{T\`\uhorn \, kh\'oa}
  \def\bibname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
  \def\chaptername{Ch\uhorn \ohorn ng}%
  \def\appendixname{Ph\d{u} l\d{u}c}%
  \def\contentsname{M\d{u}c l\d{u}c}%
  \def\listfigurename{Danh s\'ach h\`inh v\~e}%
  \def\listtablename{Danh s\'ach b\h{a}ng}%
  \def\indexname{Ch\h{i} m\d{u}c}% 
  \def\figurename{H\`inh}%
  \def\tablename{B\h{a}ng}%
  \def\partname{Ph\`\acircumflex n}%
  \def\pagename{Trang}%
  \def\headpagename{Trang}%
  \def\seename{Xem}%
  \def\alsoname{Xem th\ecircumflex m}%
  \def\enclname{K\`em theo}%
  \def\ccname{C\`ung g\h\uhorn i}%
  \def\headtoname{G\h\uhorn i}%
  \def\proofname{Ch\'\uhorn ng minh}}

\providecommand\datevietnam{%
  \def\today{%
    Ng\`ay \number\day\space
    th\'ang \number\month\space
    n\abreve m \number\year}}

\providecommand\captionsenglish{%
  \def\prefacename{Preface}%
  \def\refname{References}%
  \def\abstractname{Abstract}%
  \def\bibname{Bibliography}%
  \def\chaptername{Chapter}%
  \def\appendixname{Appendix}%
  \def\contentsname{Contents}%
  \def\listfigurename{List of Figures}%
  \def\listtablename{List of Tables}%
  \def\indexname{Index}%
  \def\figurename{Figure}%
  \def\tablename{Table}%
  \def\partname{Part}%
  \def\enclname{encl}%
  \def\ccname{cc}%
  \def\headtoname{To}%
  \def\pagename{Page}%
  \def\headpagename{Page}%
  \def\prefacename{Preface}%
  \def\seename{see}%
  \def\alsoname{see also}}

\providecommand\dateenglish{%
  \def\today{%
    \ifcase\day\or 1st\or 2nd\or 3rd\or 4th\or 5th\or 6th\or 7th\or
    8th\or 9th\or 10th\or 11th\or 12th\or 13th\or 14th\or 15th\or
    16th\or 17th\or 18th\or 19th\or 20th\or 21st\or 22nd\or 23rd\or
    24th\or 25th\or 26th\or 27th\or 28th\or 29th\or 30th\or 31st\fi
    ~\ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space
    \number\year}}

\providecommand\dateUSenglish{%
  \def\today{%
    \ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space\number\day, \number\year}}

\endinput

% end of vncaps.tex

